The temperature of the diffuse HI in the Milky Way I: High resolution HI 21 cm absorption studies

We have carried out deep, high velocity resolution, interferometric Galactic HI 21 cm absorption spectroscopy towards 32 compact extra-galactic radio sources with the Giant Metrewave Radio Telescope (GMRT) and the Westerbork Synthesis Radio Telescope (WSRT). The optical depth spectra for most sources have root mean square noise values \lesssim 10^{-3} per 1 km/s velocity channel and are thus sufficiently sensitive to detect absorption by warm neutral hydrogen with HI column densities N_HI \gtrsim 10^{20} cm^{-2}, spin temperatures T_s \leq 5000 K, and line widths equal to the thermal width (20 km/s). HI 21 cm absorption was detected against all background sources but one, B0438-436. The spectra of sources observed separately with GMRT and WSRT show excellent agreement, indicating that spectral baseline problems and contamination from HI 21 cm emission are negligible. This paper presents the absorption spectra, the emission spectra along neighbouring sightlines from the Leiden-Argentine-Bonn survey, and the derived spin temperature spectra. On every sightline, the maximum spin temperature detected (at \ge 3 sigma significance) even at a velocity resolution of 1 km/s is \gtrsim 1000 K, indicating that we are detecting the warm neutral medium along most sightlines. This is by far the largest sample of Galactic HI 21 cm absorption spectra of this quality, providing a sensitive probe of physical conditions in the neutral atomic ISM.

==> readme <==
%auto-ignore

This file contain information regarding the paper "The temperature of the diffuse HI in the Milky Way I: High resolution HI 21 cm absorption studies"

Authors: Nirupam Roy, Nissim Kanekar, Robert Braun and Jayaram N. Chengalur 

Comments: 14 pages, 5 figures. Accepted for publication in MNRAS. The definitive version will be available at http://mnras.oxfordjournals.org/

The contact details of the first author are as follows
Nirupam Roy
email  : nirupam@mpifr-bonn.mpg.de
Address: Max-Planck-Institut fur Radioastronomie,
         Auf dem Hugel 69, D-53121 Bonn, Germany
Tel    : +49 228 525491

Abstract: We have carried out deep, high velocity resolution, interferometric Galactic HI 21 cm absorption spectroscopy towards 32 compact extra-galactic radio sources with the Giant Metrewave Radio Telescope (GMRT) and the Westerbork Synthesis Radio Telescope (WSRT). The optical depth spectra for most sources have root mean square noise values \lesssim 10^{-3} per 1 km/s velocity channel and are thus sufficiently sensitive to detect absorption by warm neutral hydrogen with HI column densities N_HI \gtrsim 10^{20} cm^{-2}, spin temperatures T_s \leq 5000 K, and line widths equal to the thermal width (20 km/s). HI 21 cm absorption was detected against all background sources but one, B0438-436. The spectra of sources observed separately with GMRT and WSRT show excellent agreement, indicating that spectral baseline problems and contamination from HI 21 cm emission are negligible. This paper presents the absorption spectra, the emission spectra along neighbouring sightlines from the Leiden-Argentine-Bonn survey, and the derived spin temperature spectra. On every sightline, the maximum spin temperature detected (at \ge 3\sigma significance) even at a velocity resolution of 1 km/s is \gtrsim 1000 K, indicating that we are detecting the warm neutral medium along most sightlines. This is by far the largest sample of Galactic HI 21 cm absorption spectra of this quality, providing a sensitive probe of physical conditions in the neutral atomic ISM.


